Deep Image Prior

Deep convolutional networks have become a popular tool for image generation and restoration. Generally, their excellent performance is imputed to their ability to learn realistic image priors from a large number of example images. In this paper, we show that, on the contrary, the structure of a generator network is sufficient to capture a great deal of low-level image statistics prior to any learning. In order to do so, we show that a randomly-initialized neural network can be used as a handcrafted prior with excellent results in standard inverse problems such as denoising, super-resolution, and inpainting. Furthermore, the same prior can be used to invert deep neural representations to diagnose them, and to restore images based on flash-no flash input pairs. Apart from its diverse applications, our approach highlights the inductive bias captured by standard generator network architectures. It also bridges the gap between two very popular families of image restoration methods: learning-based methods using deep convolutional networks and learning-free methods based on handcrafted image priors such as self-similarity. Code and supplementary material are available at https://dmitryulyanov.github.io/deep_image_prior .

==> scratch.tex <==


%But why do ConvNets initially designed to perform recognition tasks~\cite{LeCun89} work so well for image restoration and generation?

%State-of-the-art ConvNets for image generation are almost invariably trained in a supervised manner on large datasets of corrupted images. One may thus assume that their excellent performance is due to their ability to learn the inversion of the degradation process from large amounts of example data. In this work, we show that, on the contrary, the excellent performance of ConvNets in such problems is in large part explained by their architecture rather than by any learned capability.


% \begin{figure*}[h]
%     \centering
%     % \deflen{mylength}{0.138\linewidth}
%     \deflen{mylengthh}{0.138\linewidth}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_0.980000p_masked}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{./inpainting/kate/kate_voronoi.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp1}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp2}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp4}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp5}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/losses_inpainting_p0.980000}.eps}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%      \vspace*{-1mm}\caption{\textbf{Reconstruction from 2\% of pixels.} \textbf{(a)} Corrupted image; \textbf{(b)}: 1-nearest neighbor interpolation (Voronoi diagram); \textbf{(c)} -- \textbf{(f)}: reconstructions with our method varying network architectures: \textbf{(c)} Encoder-decoder with bilinear upsampling; \textbf{(d)} Encoder-decoder with nearest neighbor upsampling; \textbf{(e)} UNET; \textbf{(f)} ResNet. Our method is tunable and different architectures lead to different inpainting results, yet each converges to a local minima of the data term \textbf{(g)}.}\label{fig:inpainting_sparse}%
% \end{figure*}


% \begin{figure*}
% \centering
% \begin{subfigure}[b]{0.56\linewidth}%\hspace*{15mm}
% 	\centering
%     \includegraphics[width=0.8\linewidth]{./learning_curves.eps}
% \end{subfigure}
% \begin{subfigure}[b]{0.33\linewidth}%\hspace*{15mm}
% 	\centering
%     \includegraphics[width=0.8\linewidth]{./bill.jpg}
% \end{subfigure}\\\vspace*{3mm}
% \begin{subfigure}[b]{0.56\linewidth}%\hspace*{15mm}
% 	\centering
%     \includegraphics[width=0.8\linewidth]{./learning_curves_2.eps}
% \end{subfigure}
% \begin{subfigure}[b]{0.33\linewidth}%\hspace*{15mm}
% 	\centering
%     \includegraphics[width=0.8\linewidth]{./barbara.jpg}
% \end{subfigure}

% %\vspace*{-1mm}
% \caption{Learning curves for the reconstruction task using: a natural image, the same plus i.i.d.\ noise, the same randomly scrambled, and white noise. Naturally-looking images result in much faster convergence, whereas noise is rejected.}\label{fig:recon}%\vspace*{-1mm}
% \end{figure*}


% 1800 it with 0.99 alpha

% \todo{PSNR}
% \cref{fig:jpeg}
% \cref{fig:denoising}

 % \begin{figure*}[t]
%     \centering
%     % \hspace*{-2mm}%
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{butterfly_GT.jpg}
%         % \vspace*{-6mm}\caption{Corrupted.}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{butterfly_bicubic.jpg}
%         % \vspace*{-6mm}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{butterfly_ours.jpg}
%         % \vspace*{-6mm}
%   \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{butterfly_LapSRN.jpg}
%         % \vspace*{-6mm}\caption{Baseline 2.}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{butterfly_SRResNet-MSE.jpg}
%     \end{subfigure}
%     \\
%     \centering
%     % \hspace*{-2mm}%
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{man_GT.jpg}
%         \vspace*{-6mm}\caption{Ground truth}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{man_bicubic.jpg}
%         \vspace*{-6mm}\caption{Bicubic, \textbf{Not trained}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{man_ours.jpg}
%         \vspace*{-6mm}\caption{Ours, \textbf{Not trained}}
%   \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{man_LapSRN.jpg}
%         \vspace*{-6mm}\caption{LapSRN~\cite{Lai17sr}, \textbf{Trained}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.195\linewidth}
%         \includegraphics[width=\linewidth]{man_SRResNet-MSE.jpg}
%         \vspace*{-6mm}\caption{SRResNet, \textbf{Trained}}
%     \end{subfigure}%
%     \vspace*{-1mm}\caption{\textbf{4x image super-resolution.} Similarly to e.g.\ bicubic upsampling, our method never has access to any data other than a single low-resolution image, and yet it produces much cleaner results with sharp edges close to state-of-the-art super-resolution methods (LapSRN, SRResNet) which utilize networks trained from large datasets.}\label{fig:sr}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \deflen{fourlennsr}{0.194\linewidth}
%     \renewcommand\makespy[1]{%
%         \begin{tikzpicture}[spy using outlines={rectangle,magnification=3, height=4.5cm, width=8.75cm, every spy on node/.append style={line width=2mm}}]
%                 \node (nd1){\includegraphics{#1}};
%                 \RelativeSpy{nd1-spy1}{nd1}{(0.14,0.195)}{(0.253,-0.13)}{red}
%                  \RelativeSpy{nd1-spy4}{nd1}{(0.095,0.945)}{(0.750,-0.13)}{blue}
%         \end{tikzpicture}%
%     }
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \begin{tikzpicture}[]
%                 \node (nd1){\includegraphics{butterfly_GT.jpg}};
%             \end{tikzpicture}%
%         }%
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \begin{tikzpicture}[]
%                 \node (nd1){\includegraphics{butterfly_bicubic.jpg}};
%             \end{tikzpicture}%
%         }%
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \begin{tikzpicture}[]
%                 \node (nd1){\includegraphics{butterfly_ours.jpg}};
%             \end{tikzpicture}%
%         }%
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \begin{tikzpicture}[]
%                 \node (nd1){\includegraphics{butterfly_LapSRN.jpg}};
%             \end{tikzpicture}%
%         }%
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \begin{tikzpicture}[]
%                 \node (nd1){\includegraphics{butterfly_SRResNet-MSE.jpg}};
%             \end{tikzpicture}%
%         }%
%     \end{subfigure}%
%     \\%
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \makespy{man_GT.jpg}
%         }
%         % \vspace*{-1mm}
%         \caption{Original image}
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \makespy{man_bicubic.jpg}
%         }
%         % \vspace*{-1mm}
%         \caption{Bicubic, \textbf{Not trained}}
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \makespy{man_ours.jpg}
%         }
%         % \vspace*{-1mm}
%         \caption{Ours, \textbf{Not trained}}
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%            \makespy{man_LapSRN.jpg}
%         }
%         % \vspace*{-1mm}
%         \caption{LapSRN, \textbf{Trained}}
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \resizebox{1.00\linewidth}{!}{
%             \makespy{man_SRResNet-MSE.jpg}
%         }
%         % \vspace*{-1mm}
%         \caption{SRResNet, \textbf{Trained}}
%     \end{subfigure}%
%     \caption{\textbf{4x image super-resolution.} Similarly to e.g.\ bicubic upsampling, our method never has access to any data other than a single low-resolution image, and yet it produces much cleaner results with sharp edges close to state-of-the-art super-resolution methods (LapSRN~\cite{Lai17sr}, SRResNet~\cite{Ledig17sr}) which utilize networks trained from large datasets.}\label{fig:sr}
% \end{figure*}

    % \newcommand\makespy[0]{%
    %       % \RelativeSpy{nd1-spy1}{nd1}{(0.1,0.60)}{(0.145,-0.140)}{red}
    %       % \RelativeSpy{nd1-spy2}{nd1}{(0.68,0.38)}{(0.445,-0.140)}{yellow}
    %       % \RelativeSpy{nd1-spy3}{nd1}{(0.1,0.38)}{(0.745,-0.140)}{blue}
    %       % \RelativeSpy{nd1-spy4}{nd1}{(0.68,0.15)}{(1.045,-0.140)}{green}

    %       \RelativeSpy{nd1-spy1}{nd1}{(0.1,0.60)}{(0.157,-0.150)}{red}
    %       \RelativeSpy{nd1-spy2}{nd1}{(0.68,0.38)}{(0.485,-0.150)}{yellow}
    %       % \RelativeSpy{nd1-spy3}{nd1}{(0.1,0.38)}{(0.775,-0.150)}{blue}
    %       \RelativeSpy{nd1-spy4}{nd1}{(0.68,0.15)}{(0.800,-0.150)}{green}
    % }

% \renewcommand\makespy[1]{%
%     \includegraphics[width=\textwidth]{#1}
% }%


%     \renewcommand\makespy[1]{%

    %     \begin{tikzpicture}[spy using outlines={rectangle,magnification=1.7, height=1.5cm, width=2.95cm, every spy on node/.append style={line width=0.75mm}}]
    %             \node (nd1){\includegraphics{#1}};

    %             \RelativeSpy{nd1-spy1}{nd1}{(0.57,0.355)}{(0.167,-0.08)}{yellow}
    %             \RelativeSpy{nd1-spy2}{nd1}{(0.78,0.575)}{(0.5,-0.08)}{blue}
    %             \RelativeSpy{nd1-spy4}{nd1}{(0.50,0.714)}{(0.833,-0.08)}{green}
    %     \end{tikzpicture}
    % }



    % \begin{subfigure}[b]{\fourlenneew}
    %     \resizebox{\textwidth}{!}{
    %         \makespy{./Cameraman256_orig.jpg}
    %     }
    %     \vspace*{-4mm}
    %     \caption{Original image}
    % \end{subfigure}
    % \begin{subfigure}[b]{\fourlenneew}
    %     \resizebox{\linewidth}{!}{
    %         \makespy{./Cameraman256_masked.jpg}
    %     }
    %     \vspace*{-4mm}\caption{Corrupted image}
    % \end{subfigure}
    % \begin{subfigure}[b]{\fourlenneew}
    %     \resizebox{\linewidth}{!}{
    %         \makespy{./Cameraman256_papyan.jpg}
    %     }
    %     \vspace*{-4mm}  \caption{\cite{PapyanRSE17}}
    % \end{subfigure}
    % \begin{subfigure}[b]{\fourlenneew}
    %     \resizebox{\linewidth}{!}{
    %         \makespy{./Cameraman256_ours.jpg}
    %     }
    %     \vspace*{-4mm}\caption{Deep Image Prior}
    % \end{subfigure}\\
    %\vspace{-4mm}



    %\vspace*{-1mm}
    % \caption{Comparison between our method and the algorithm in~\cite{PapyanRSE17}. See \cref{fig:shepard} bottom row for visual comparison.}\label{tab:papyan}




% \begin{figure*}[h]
%     \centering
%     % \deflen{mylength}{0.138\linewidth}
%     \deflen{mylengthh}{0.138\linewidth}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_0.980000p_masked}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{./inpainting/kate/kate_voronoi.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp1}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp2}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp4}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/kate_inpainting-p0.980000_exp5}.jpg}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{\mylengthh}
%         \includegraphics[width=\linewidth]{{./inpainting/kate/losses_inpainting_p0.980000}.eps}
%         \vspace*{-6mm}\caption{}
%     \end{subfigure}
%      \vspace*{-1mm}\caption{\textbf{Reconstruction from 2\% of pixels.} \textbf{(a)} Corrupted image; \textbf{(b)}: 1-nearest neighbor interpolation (Voronoi diagram); \textbf{(c)} -- \textbf{(f)}: reconstructions with our method varying network architectures: \textbf{(c)} Encoder-decoder with bilinear upsampling; \textbf{(d)} Encoder-decoder with nearest neighbor upsampling; \textbf{(e)} UNET; \textbf{(f)} ResNet. Our method is tunable and different architectures lead to different inpainting results, yet each converges to a local minima of the data term \textbf{(g)}.}\label{fig:inpainting_sparse}%
% \end{figure*}





% \begin{figure}[h]
%     \centering
%     \hspace*{-2mm}\begin{subfigure}[b]{0.5\linewidth}
%         \includegraphics[width=\linewidth]{{./inpainting/2p/losses_inpainting_p0.980000}.eps}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.5\linewidth}
%         \includegraphics[width=\linewidth]{{./inpainting/05p/losses_inpainting_p0.995000}.eps}
%     \end{subfigure}
%     \vspace*{-1mm}\caption{\textbf{Optimization losses for examples (b) -- (e) from fig \ref{fig:inpainting_sparse}.} Left image for the first row and the right for the second. Dashed and solid lines show MSE loss calculated using only known pixels and all pixels respectively. We see that with every network architecture (b) -- (e) the optimization loss (dashed) goes down, while the difference between the generated image and ground truth (solid) is very different.}\label{fig:inpainting_sparse_plot}
% \end{figure}

 %\section{Natural pre-image}\label{s:inversion}

% \begin{figure}[h]
% \makebox[.14\linewidth]{conv1}%
% \makebox[.14\linewidth]{conv2}%
% \makebox[.14\linewidth]{conv3}%
% \makebox[.14\linewidth]{conv4}%
% \makebox[.14\linewidth]{conv5}%
% \makebox[.14\linewidth]{fc6}%
% \makebox[.14\linewidth]{fc7}
% \centering\includegraphics[width=1\linewidth,clip,trim={0 515em 0 0em}]{..jpg}
% \caption{\textbf{AlexNet feature inversion.} Each group of two rows shows the result of inverting a different layer of AlexNet for different refence images. In each group, the top row is the inversion obtained using our structural regularizer, whereas the bottom row is the method of~\cite{mahendran15understanding}. While both methods do not make use of regularizers which are \emph{not} learned from data, our approach recovers dramatically more natural inversions.}\label{fig:inv}
% \end{figure}

 % \begin{table*}[h]

%     %\vspace*{-0.2cm}
% \end{table*}


% % \begin{table*}[h]
% %     \centering
% %     \begin{tabular}{@{}lccccccccccc@{}}\toprule
% %                               & \small{Barbara}  & \small{Boat}  & \small{House} & \small{Lena} & \small{Peppers} & \small{C.man} & \small{Couple} & \small{Finger}& \small{Hill}     & \small{Man}   & \small{Montage} \\ \midrule
% %         \small{Papyan et al.} & 28.14            & 31.44         & 34.58         & 35.04        & {29.91}         & 27.90          & 31.18         & 31.34                 & 32.35            & 31.92         & 28.05   \\
% %         \small{Ours}      & \textbf{30.88}   & \textbf{32.84}& \textbf{37.52}&\textbf{36.05}&\textbf{31.22}   &\textbf{28.83}  &\textbf{32.43} &\textbf{34.40}                      & \textbf{33.15}   & \textbf{32.26}& \textbf{29.85}  \\ \bottomrule
% %     \end{tabular}
% %     \caption{Comparison between our method and the algorithm in~\cite{PapyanRSE17}. See \cref{fig:shepard} bottom row for visual comparison.}\label{tab:papyan}
% %     \vspace{-0.3cm}
% % \end{table*}

%  \newcommand\makerow[3]{%
%     \centering
%     \begin{subfigure}[b]{\fourlennsr}
%         \makespy{./#1/#2_GT.jpg}
%         \IfEqCase{#3}{%
%             {1}{\vspace*{-6mm}\caption{Original image \\ \quad}}%
%         }
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \makespy{./#1/#2_bicubic.jpg}
%         \IfEqCase{#3}{%
%             {1}{\vspace*{-6mm}\caption{Bicubic, \\ \textbf{Not trained}}}%
%         }
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \makespy{{./#1/#2_deep_prior}.jpg}
%         \IfEqCase{#3}{%
%             {1}{\vspace*{-6mm}\caption{Ours, \\ \textbf{Not trained}}}%
%         }
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \makespy{./#1/#2_LapSRN.jpg}
%         \IfEqCase{#3}{%
%             {1}{\vspace*{-6mm}\caption{LapSRN, \\ \textbf{trained}}}%
%         }
%     \end{subfigure}
%     \begin{subfigure}[b]{\fourlennsr}
%         \makespy{./#1/#2_VDSR.jpg}
%         \IfEqCase{#3}{%
%             {1}{\vspace*{-6mm}\caption{VDSR, \\ \textbf{Trained}}}%
%         }
%     \end{subfigure}
% }%

% \begin{figure*}[t]
%     \centering
%     % \makerow{x8}{butterfly}{0} \\ \vspace*{-4mm}
%     \makerow{x8}{bird}{0} \\ \vspace*{-4mm}
%     \makerow{x8}{baby}{1}
%     % \makerow{x8}{head}{0} \\ \vspace*{-4mm}
%     % \makerow{x8}{woman}{1}
%     \caption{\textbf{8x image super-resolution.} Comparison on the Set5 dataset.}\label{fig:sr8x}
% \end{figure*}


% \begin{figure}[h]
%     \centering
%     \hspace*{-2mm}\begin{subfigure}[b]{0.5\linewidth}
%         \includegraphics[width=\linewidth]{{./inpainting/2p/losses_inpainting_p0.980000}.eps}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.5\linewidth}
%         \includegraphics[width=\linewidth]{{./inpainting/05p/losses_inpainting_p0.995000}.eps}
%     \end{subfigure}
%     \vspace*{-1mm}\caption{\textbf{Optimization losses for examples (b) -- (e) from fig \ref{fig:inpainting_sparse}.} Left image for the first row and the right for the second. Dashed and solid lines show MSE loss calculated using only known pixels and all pixels respectively. We see that with every network architecture (b) -- (e) the optimization loss (dashed) goes down, while the difference between the generated image and ground truth (solid) is very different.}\label{fig:inpainting_sparse_plot}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \deflen{twolenn}{0.48\linewidth}
%     \renewcommand\makespy[1]{%

%         \begin{tikzpicture}[spy using outlines={rectangle,magnification=2.7, height=2.7cm, width=6.6cm, every spy on node/.append style={ultra thin}}]
%                 \node (nd1){\includegraphics{#1}};

%                 \RelativeSpy{nd1-spy1}{nd1}{(0.37,0.355)}{(0.253,-0.12)}{green}
%                 % % \RelativeSpy{nd1-spy2}{nd1}{(0.68,0.575)}{(0.5,-0.13)}{blue}
%                 \RelativeSpy{nd1-spy4}{nd1}{(0.87,0.694)}{(0.736,-0.12)}{blue}
%         \end{tikzpicture}
%     }
%     \begin{subfigure}[b]{\twolenn}
%         \resizebox{\textwidth}{!}{
%             \makespy{jpeged.jpg}
%         }
%         \vspace*{-6mm}
%         \caption{Corrupted image}
%     \end{subfigure}
%     \begin{subfigure}[b]{\twolenn}
%         \resizebox{\linewidth}{!}{
%             \makespy{restored.jpg}
%         }
%         \vspace*{-6mm}\caption{Restored image}
%     \end{subfigure}
%     \vspace*{-2mm}
%     \caption{\textbf{JPEG artifacts removal.} Our method can be applied to noise of any type.}\label{fig:jpeg}
% \end{figure}



% \centering
    % % \deflen{mylengthoop}{0.193\linewidth}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{._ench2x_32_padded}.jpg}
    %     % \caption{Ours}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-219}.jpg}
    %     % \caption{LCIS}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-221}.jpg}
    %     % \caption{WLS}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-222}.jpg}
    %     % \caption{TV}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-223}.jpg}
    %     % \caption{L0}
    % \end{subfigure}\\
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{._ench_32_lf_padded}.jpg}
    %     \caption{Ours}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-236}.jpg}
    %     \caption{LCIS~\cite{tumblin99lcis}}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-238}.jpg}
    %     \caption{WLS~\cite{farbman2008boosting}}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-239}.jpg}
    %     \caption{TV\cite{rudin1992tv}}
    % \end{subfigure}
    % \begin{subfigure}[h]{\mylengthoop}
    %     \includegraphics[width=\linewidth]{{./Page-9-Image-240}.jpg}
    %     \caption{L0 smoothing~\cite{xu2011l0smoothing}}
    % \end{subfigure}%
    %  %\vspace*{-1mm}
    %  \caption{\textbf{High frequency boosting.} The coarse approximations of the image are shown in the bottom row while boosted versions in the top one. \todo{evaluate}. The images for methods in comparion are taken directly from~\cite{xu2011l0smoothing}. }\label{fig:enchancement_comparison}


% We compare our boosting results to other methods in~\cref{fig:enchancement_comparison}. While we use a simple L2 reconstruction loss, deep image prior can be combined with the objectives of any smoothing method.


% WLS~\cite{farbman2008boosting}
% reconusing the objective () the image is gradually reconstructed reconstructed for observe We observe, that the iamg
 % \begin{figure}[t]
%     \centering
%     \deflen{twoen}{0.48\linewidth}
%     \newcommand\makespy[1]{%

%         \begin{tikzpicture}[spy using outlines={rectangle,magnification=2.7, height=3.0cm, width=5.9cm, every spy on node/.append style={ultra thin}}]
%                 \node (nd1){\includegraphics{#1}};

%                 \RelativeSpy{nd1-spy1}{nd1}{(0.37,0.355)}{(0.167,-0.08)}{yellow}
%                 \RelativeSpy{nd1-spy2}{nd1}{(0.68,0.575)}{(0.5,-0.08)}{blue}
%                 \RelativeSpy{nd1-spy4}{nd1}{(0.90,0.694)}{(0.833,-0.08)}{green}
%         \end{tikzpicture}
%     }
%     \begin{subfigure}[b]{\twolen}
%         \resizebox{\textwidth}{!}{
%             \makespy{cave01_ours.jpg}
%         }
%         \vspace*{-6mm}
%         \caption{Original image.}
%     \end{subfigure}
%     \begin{subfigure}[b]{\twolen}
%         \resizebox{\linewidth}{!}{
%             \makespy{barbara_masked.jpg}
%         }
%         \vspace*{-6mm}\caption{Corrupted image.}
%     \end{subfigure}
%     \vspace*{-6mm}
%     \caption{Restoration quality for an image with 50\% of pixel values being unknown. Both our method and the method of Papyan et al.~\cite{PapyanRSE17} use only corrupted image for reconstruction, yet quality of our method is higher. See table \cref{tab:papyan} for quantitative comparison.}\label{fig:papyan}
% \end{figure*}


%In the domain of image recognition, the work~\cite{zhang16understanding} has recently demonstrated that a standard image classification network can fit perfectly well a large training set of images with random labels. This extreme overfitting capacity means that the excellent generalization performance of classification ConvNets observed in practice is at least in part due to their architecture that can self-regulate the use of the vast capacity. Our work demonstrates an analogous effect for generative ConvNets.

% Self-sim based methods (NLMeans, BM3D), Irani works do not require learning, and thus do not require a dataset of statistically similar clean or degraded images. However self-similarity invariably relies on l2-pix similarity and is essentially flat.. Also might be slow (TODO: CHECK!!). Lefkimmiatis~\cite{Lefkimmiatis17} combines ConvNets and self-similarity search but still requires training on a large number of noise-corrupted images.

% Sparse dictionary learning and convolutional sparse coding is another group of related works. Usually flat. Few non-flat variants including DeconvNets are trained by layer-wise training, which is quite different from ours.
